An Efficient Real Time DDoS Detection Model Using Machine Learning Algorithms

Distributed Denial of Service attacks have become a significant threat to industries and governments leading to substantial financial losses. With the growing reliance on internet services, DDoS attacks can disrupt services by overwhelming servers with false traffic causing downtime and data breaches. Although various detection techniques exist, selecting an effective method remains challenging due to trade-offs between time efficiency and accuracy. This research focuses on developing an efficient real-time DDoS detection system using machine learning algorithms leveraging the UNB CICDDoS2019 dataset including various traffic features. The study aims to classify DDoS and non-DDoS traffic through various ML classifiers including Logistic Regression, K-Nearest Neighbors, Random Forest, Support Vector Machine, Naive Bayes. The dataset is preprocessed through data cleaning, standardization and feature selection techniques using Principal Component Analysis. The research explores the performance of these algorithms in terms of precision, recall and F1-score as well as time complexity to create a reliable system capable of real-time detection and mitigation of DDoS attacks. The findings indicate that RF, AdaBoost and XGBoost outperform other algorithms in accuracy and efficiency, making them ideal candidates for real-time applications.

==> An_Efficient_Real_Time_DDoS_Detection_Model_Using_Machine_Learning_Algorithms/refs_.tex <==
@article{aa1,
  title={Enhanced neurologic concept recognition using a named entity recognition model based on transformers},
  author={Azizi, Sima and Hier, Daniel B and Wunsch II, Donald C},
  journal={Frontiers in Digital Health},
  volume={4},
  pages={1065581},
  year={2022},
  publisher={Frontiers}
}
@article{b1,
  title={Natural language processing for smart healthcare},
  author={Zhou, Binggui and Yang, Guanghua and Shi, Zheng and Ma, Shaodan},
  journal={IEEE Reviews in Biomedical Engineering},
  year={2022},
  publisher={IEEE}
}

@article{b2,
  title={Using Natural Language Processing and Machine Learning to Preoperatively Predict Lymph Node Metastasis for Non--Small Cell Lung Cancer With Electronic Medical Records: Development and Validation Study},
  author={Hu, Danqing and Li, Shaolei and Zhang, Huanyao and Wu, Nan and Lu, Xudong},
  journal={JMIR Medical Informatics},
  volume={10},
  number={4},
  pages={e35475},
  year={2022},
  publisher={JMIR Publications Toronto, Canada}
}
@inproceedings{b3,
  title={Using natural language processing to classify serious illness communication with oncology patients},
  author={Davoudi, Anahita and Tissot, Hegler and Doucette, Abigail and Gabriel, Peter E and Parikh, Ravi and Mowery, Danielle L and Miranda, Stephen P},
  booktitle={AMIA Annual Symposium Proceedings},
  volume={2022},
  pages={168},
  year={2022},
  organization={American Medical Informatics Association}
}

@article{bbc,
  title={A deep language model for symptom extraction from clinical text and its application to extract covid-19 symptoms from social media},
  author={Luo, Xiao and Gandhi, Priyanka and Storey, Susan and Huang, Kun},
  journal={IEEE Journal of Biomedical and Health Informatics},
  volume={26},
  number={4},
  pages={1737--1748},
  year={2021},
  publisher={IEEE}
}

@inproceedings{bci,
  title={Disease prediction from speech using natural language processing and deep learning method},
  author={Kumar, Rahul and Pradhan, Sushant and Rebaka, Tejaswi and Prakash, Jay},
  booktitle={Congress on Intelligent Systems: Proceedings of CIS 2020, Volume 2},
  pages={407--413},
  year={2021},
  organization={Springer}
}

@inproceedings{bbci,
  title={Automated question-answer medical model based on deep learning technology},
  author={Abdallah, Abdelrahman and Kasem, Mahmoud and Hamada, Mohamed A and Sdeek, Shaymaa},
  booktitle={Proceedings of the 6th International Conference on Engineering \& MIS 2020},
  pages={1--8},
  year={2020}
}
 
@article{b4,
  title={Text messaging-based medical diagnosis using natural language processing and fuzzy logic},
  author={Omoregbe, Nicholas AI and Ndaman, Israel O and Misra, Sanjay and Abayomi-Alli, Olusola O and Dama{\v{s}}evi{\v{c}}ius, Robertas and Dogra, Ayush},
  journal={Journal of Healthcare Engineering},
  volume={2020},
  pages={1--14},
  year={2020},
  publisher={Hindawi Limited}
}

@article{b6,
  title={Clinical text data in machine learning: systematic review},
  author={Spasic, Irena and Nenadic, Goran and others},
  journal={JMIR medical informatics},
  volume={8},
  number={3},
  pages={e17984},
  year={2020},
  publisher={JMIR Publications Inc., Toronto, Canada}
}

@article{b7,
  title={Natural language processing of clinical notes on chronic diseases: systematic review},
  author={Sheikhalishahi, Seyedmostafa and Miotto, Riccardo and Dudley, Joel T and Lavelli, Alberto and Rinaldi, Fabio and Osmani, Venet and others},
  journal={JMIR medical informatics},
  volume={7},
  number={2},
  pages={e12239},
  year={2019},
  publisher={JMIR Publications Inc., Toronto, Canada}
}

@article{b8,
  title={Deep learning approaches for predicting glaucoma progression using electronic health records and natural language processing},
  author={Wang, Sophia Y and Tseng, Benjamin and Hernandez-Boussard, Tina},
  journal={Ophthalmology Science},
  volume={2},
  number={2},
  pages={100127},
  year={2022},
  publisher={Elsevier}
}
@inproceedings{b9,
  title={Symptoms Based Disease Prediction from Bengali Text Using Transformer Network Based Pretrained Model},
  author={Hossain, Md Mamun and Mou, Munira Akter and Oishi, Mst Najmun Nahar},
  booktitle={2022 25th International Conference on Computer and Information Technology (ICCIT)},
  pages={575--580},
  year={2022},
  organization={IEEE}
}

@article{bb1,
  title={Text messaging-based medical diagnosis using natural language processing and fuzzy logic},
  author={Omoregbe, Nicholas AI and Ndaman, Israel O and Misra, Sanjay and Abayomi-Alli, Olusola O and Dama{\v{s}}evi{\v{c}}ius, Robertas and Dogra, Ayush},
  journal={Journal of Healthcare Engineering},
  volume={2020},
  pages={1--14},
  year={2020},
  publisher={Hindawi Limited}
}

@article{bb2,
title = {Prediction and evaluation of combination pharmacotherapy using natural language processing, machine learning and patient electronic health records},
journal = {Journal of Biomedical Informatics},
volume = {133},
pages = {104164},
year = {2022},
issn = {1532-0464},
doi = {https://doi.org/10.1016/j.jbi.2022.104164},
url = {https://www.sciencedirect.com/science/article/pii/S1532046422001769},
author = {Pingjian Ding and Yiheng Pan and Quanqiu Wang and Rong Xu}
}
 
@article{bb3,
  title={Natural language processing in psychiatry: the promises and perils of a transformative approach},
  author={Rezaii, Neguine and Wolff, Phillip and Price, Bruce H},
  journal={The British Journal of Psychiatry},
  volume={220},
  number={5},
  pages={251--253},
  year={2022},
  publisher={Cambridge University Press}
}

@article{b5,
  title={Novel use of natural language processing (NLP) to predict suicidal ideation and psychiatric symptoms in a text-based mental health intervention in Madrid},
  author={Cook, Benjamin L and Progovac, Ana M and Chen, Pei and Mullin, Brian and Hou, Sherry and Baca-Garcia, Enrique and others},
  journal={Computational and mathematical methods in medicine},
  volume={2016},
  year={2016},
  publisher={Hindawi}
}
@misc{n, title={Symptom2disease}, url={https://www.kaggle.com/datasets/niyarrbarman/symptom2disease}, journal={Kaggle}, author={Barman, Niyar R}, year={2023}, month={Apr}} 

 
